Intriguing Properties of Contrastive Losses

We study three intriguing properties of contrastive learning. First, we generalize the standard contrastive loss to a broader family of losses, and we find that various instantiations of the generalized loss perform similarly under the presence of a multi-layer non-linear projection head. Second, we study if instance-based contrastive learning (with a global image representation) can learn well on images with multiple objects present. We find that meaningful hierarchical local features can be learned despite the fact that these objectives operate on global instance-level features. Finally, we study the phenomenon of feature suppression among competing features shared across augmented views, such as "color distribution" vs "object class". We construct datasets with explicit and controllable competing features, and show that, for contrastive learning, a few bits of easy-to-learn shared features can suppress, and even fully prevent, the learning of other sets of competing features. In scenarios where there are multiple objects in an image, the dominant object would suppress the learning of smaller objects. Existing contrastive learning methods critically rely on data augmentation to favor certain sets of features over others, and could suffer from learning saturation for scenarios where existing augmentations cannot fully address the feature suppression. This poses open challenges to existing contrastive learning techniques.

==> content/abstract.tex <==
\begin{abstract}
%Contrastive loss and its variants have become very popular recently for learning visual representations without supervision. 
%In this work, 
We study three intriguing properties of contrastive learning. 
First, we generalize the standard contrastive loss to a broader family of losses, and we find that various instantiations of the generalized loss perform similarly under the presence of a multi-layer non-linear projection head.
Second, we study if instance-based contrastive learning (with a global image representation) can learn well on images with multiple objects present. We find that meaningful hierarchical local features can be learned despite the fact that these objectives operate on global instance-level features. 
Finally, we study the phenomenon of \textit{feature suppression} among competing features shared across augmented views, such as ``color distribution'' vs ``object class''. We construct datasets with explicit and controllable competing features, and show that, for contrastive learning, a few bits of easy-to-learn shared features can suppress, and even fully prevent, the learning of other sets of competing features.
In scenarios where there are multiple objects in an image, the dominant object would suppress the learning of smaller objects.
Existing contrastive learning methods critically rely on data augmentation to favor certain sets of features over others, and could suffer from learning saturation for scenarios where existing augmentations cannot fully address the feature suppression.
This poses open challenges to existing contrastive learning techniques~\footnote{Code and visualization at \href{https://contrastive-learning.github.io/intriguing}{https://contrastive-learning.github.io/intriguing}.}.
%~\footnote{Code at \href{https://github.com/google-research/simclr/tree/master/colabs/intriguing\_properties}{https://github.com/google-research/simclr/tree/master/colabs/intriguing\_properties}.}
\end{abstract}

==> content/conclusion.tex <==
\section{Conclusion}

In this work, we study three intriguing properties of contrastive losses. In particular, our results highlight that feature suppression is still an open challenge in contrastive learning. While there is a plethora of work on improving contrastive learning, few of them directly aim to address feature suppression. This limitation of contrastive learning becomes a bottleneck for scenarios where existing augmentation cannot fully address the feature suppression phenomenon, and learning would saturate at a level of dissatisfaction.

We would also like to point out some limitations of our study. Firstly, we focus mostly on contrastive learning with explicit negatives (e.g. SimCLR and MoCo). We believe other methods based on clustering and/or without negative pairs would exhibit similar phenomenon but we leave that as future work. Secondly, many of our proposed image datasets are not fully realistic despite being composed from some (challenging) natural image datasets such as ImageNet. We admit it is very hard to explore competing features or multiple objects in a controllable fashion on realistic large scale image datasets.

%In this work, we first generalize the standard contrastive loss to a broader family of losses, with an abstract form of $\mathcal{L}_{\text{alignment}} + \lambda \mathcal{L}_{\text{distribution}}$. We show that the regularization weight $\lambda$ is (within a range) inversely correlated to temperature $\tau$ of standard contrastive loss. With a multi-layer non-linear projection head, different variants of generalized contrastive losses perform similarly under the linear evaluation protocol. 
%We further show that the distribution losses are saturated quickly with a few bits of entropy.

%We then study the feature suppression phenomenon in contrastive learning. By constructing three datasets with explicit and controllable competing features, our experiments show that a few bits of easy-to-learn features could suppress, or even fully prevent, the learning of other sets of features. In scenarios where multiple objects exist in an image, the dominant object would suppress the learning of smaller objects. This observation persists across different instantiations of contrastive losses, model sizes and batch sizes (with or without memories), despite that it is far less significant in an autoencoder based on a reconstruction loss. 
% Potential causes and limitations of existing methods are also discussed. 

% \textbf{Why is it difficult to learn competing features?} 
% It is not entirely clear to us why a few bits of competing features could cause significant detrimental effects, but here are some conjectures. 
%The exact cause of feature suppression is not fully understood in this work and requires future research. We conjecture the following:

% \begin{itemize}[topsep=0pt, partopsep=0pt, leftmargin=15pt, parsep=0pt, itemsep=5pt]
%     \item One possibility is that the contrastive loss quickly saturates with a few bits of mutual information in hidden representations learned between two augmented views. This is because the distribution matching loss saturates quickly with a few bits of entropy (see Appendix~\ref{app:dist_sat}). Even using a huge batch size only helps at roughly log scale. However, simply reducing the loss saturation may not be enough. Our results show that increasing the batch size or using a large number of negatives buffered from an EMA network have little to none effect at preventing this detriment. % Furthermore, considering the case where identical augmentation is applied to create two views, the alignment term is always zero while only the distribution/entropy term needs to be optimized, reminiscent of autoencoder based on reconstruction, this aims to (perhaps undesirably) compress all features into latent representations.
%     \item Another possibility is that competing features divide the dataset so that it make the effective dataset size smaller. This would be evident in the extreme case, where every image has an unique ID that will not be destroyed by the augmentation. Then it would be trivial for the model to identity positive pairs correctly. When several examples share an ID, the model only needs to distinguish among these few, a smaller set compared to all examples. %Due to the instance discrimination nature of the objective (i.e. the postive pairs are from augmented views of the same example), which only requires a maximum of $\log(N)$ bits in the augmented view to solve the contrastive task, where $N$ is dataset size. However, by increasing the weighting of distribution/entropy term, this could be changed.
% \end{itemize}

%Interestingly, when applying contrastive loss to \textit{pairs of identical images}, the alignment term zeros out, and the only loss left is distribution matching loss. Considering distribution matching loss as a proxy for negative entropy, maximizing the entropy of representation $U$ is equivalent to maximizing the mutual information between data $X$ and its representation $U$ given a deterministic encoder, i.e. $H(U) = MI(X; U)$. This naturally connects to reconstruction loss in autoencoder, which is an lower bound on the $MI(X; U)$.

% \paragraph{Connection to reconstruction loss in autoencoder}

% When applying (generalized) contrastive loss to \textit{pairs of identical images}, the alignment term zeros out, and the only loss left is the distribution loss. Given that distribution loss is a proxy of entropy loss, the contrastive loss is minimized when the entropy of latent representations for the dataset is maximized. Maximizing the entropy of representation is equivalent to maximizing the mutual information between data example $x$ and the latent representation $u$ given a deterministic encoder (which makes $H(u|x)=0$ in $MI(x, u) = H(u) - H(u|x)$). 

% It is well known that reconstruction error in autoencoder is a lower bound on $MI(u, x)$. So both contrastive loss (on pairs of identical images) and reconstruction loss could be minimized, if the mutual information between data point $x$ and the representation $u$ is maximized. However, in practice, it is unlikely one could fully maximize $MI(u, x)$, and these two losses could behave very differently and lead to distinct representations.


%Our results resonate with~\cite{chen2020simple} on the importance of data augmentation for contrastive learning, as it can be used as a critical tool for favoring certain sets of competing features than the others. It also raises a question for future research: is there a better learning strategy for reducing the feature suppression effect while relying less on hand-crafted / heuristic-based augmentations?


% Furthermore, our study provides some new perspective on critical design choices made in SimCLR~\cite{chen2020simple,chen2020big}.

% \textbf{Data augmentation}. The data augmentation is a effective way to trim down the mutual information between two augmented views. For example, random crop could create views that share object identity, and color distortion could reduce the those bits of color information shared between two views. Despite that data augmentations play a critical role in contrastive learning, but it still requires a significant amount of engineering for a specific modality or dataset. Alternative approaches could further benefit the contrastive learning in general.
% It is likely the bits that agree, after effective augmentations, are those associated with object/part identity, leading to learning similar like fine-grained supervised learning. Although the mutual information bits are low after augmentations, the network will likely need to extract more features to find a few bits that agree. 

% \textbf{Projection head}. Given the loss itself quickly saturates with a few bits of mutual information, the output of the projection head has less incentive to involve more bits, which may explain why (1) a small number (e.g. 128) of dimensionality suffices to represent each image well for the loss, and (2) the former layer of the neural network is richer in representation and better suited for downstream tasks.

% \textbf{Batch size}. Although bigger batch size helps, they tend to saturate at a manageable number in practice. Given that data augmentation reduces the mutual information, it is expected that the effect of large batch size also saturates quickly. Purely relying on increasing batch size to ensure more bits to be learned has a significant limitation. Because in order to ensure 32 bits of information, it requires $2^32$ ($\sim10$ billion) batch size, and as the model scales, we would expect the representations to have more bits in representations. 


% Potential TODOs:
% * ImageNet fine-tuning
% * BYOL, SWAV exp (show clustering based methods also have similar issues)
% * using hash_id=False for all? or a comparison? (bits are smaller than they are in x-axis due to collision)


==> content/intro.tex <==
\section{Introduction}

%Contrastive learning~\cite{becker1992self,dosovitskiy2014discriminative,oord2018representation,wu2018unsupervised,hjelm2018learning,bachman2019learning,henaff2019data,tian2019contrastive,misra2019self,he2019momentum,li2020prototypical,tian2020makes,chen2020simple,chen2020big} has achieved great successes recently in learning unsupervised visual representations. 
Contrastive learning~\cite{becker1992self,dosovitskiy2014discriminative,oord2018representation,wu2018unsupervised,hjelm2018learning,bachman2019learning,henaff2019data,tian2019contrastive,misra2019self,he2019momentum,li2020prototypical,tian2020makes,chen2020simple,chen2020big} has achieved great successes recently for learning visual representations without supervision. 
As shown in~\cite{chen2020simple,chen2020big}, contrastive learning can learn representations that rival supervised learning, and significantly improve the state-of-the-art in semi-supervised learning on ImageNet.
One successful use case of contrastive loss for self-supervised learning is to make \textit{augmented} views of the same example agree~\cite{becker1992self,dosovitskiy2014discriminative,chen2020simple}. A widely used contrastive loss to encourage agreement is based on cross entropy~\cite{sohn2016improved,oord2018representation,wu2018unsupervised,chen2020simple}. Given an augmented view of an example, the contrastive prediction task aims to classify a set of candidates into the positive example (i.e. the other augmented view of the same example) and negative ones via the cross entropy loss. %Despite the success, there is little understanding of its effectiveness or potential limitations. 

In this work, to understand the effectiveness and limitation of existing contrastive learning methods, we study three intriguing aspects. First, we propose a generalization of the standard contrastive loss, and systematically study their performance differences.
% This generalization, inspired and built upon previous work~\cite{wang2020understanding}, allows a wider set of instantiations by leveraging different prior distributions. We observe that instances of this family of contrastive losses perform similarly under the presence of a multi-layer non-linear projection head.
% We show instances of this family of contrastive losses perform similarly under presences of a multi-layer non-linear projection head, and the temperature scaling ($\tau$) widely used in standard contrastive loss is inversely related to the weighting ($\lambda$) between two loss terms.
Second, we study if the instance-based contrastive learning, for which the contrastive loss operates on global representation of an input image, can learn well on images with multiple objects present, and whether or not it leads to meaningful local features.
Finally, we systematically study the feature suppression phenomenon in contrastive learning. The suppression effect occurs among competing features shared across augmented views. For example, with random cropping as the augmentation, ``color distribution'' and ``object class'' are often competing features as they are likely shared between two augmented views. The suppression effect among competing features can significantly degenerate the representation quality, or even completely disable the learning of certain features, as shown in our experiments. Existing methods critically rely on hand-crafted data augmentation to favor certain sets of competing features than others. % In other words, these features constitute of mutual information bits between two augmented views. It has been shown that the existence of competing features like ``color distribution'' can significantly reduce the effectiveness of contrastive learning~\cite{chen2020simple}.

%In order to study this phenomenon further in a quantitative manner, we construct datasets with explicit and controllable competing features. Our experiments show that shared features that are easy-to-learn, even when they only constitute a few bits of mutual information, could suppress, and even fully prevent, the learning of other sets of features. 
%This phenomenon persists across different instantiations of the generalized contrastive loss, model sizes, as well as batch sizes (with or without memory), despite that it is much less detrimental in autoencoders based on a reconstruction loss. We discuss some potential reasons that lead to the phenomenon, and note that existing contrastive learning methods~\cite{dosovitskiy2014discriminative,bachman2019learning,he2019momentum,chen2020simple,grill2020bootstrap} critically rely on hand-crafted data augmentation to favor certain sets of competing features than others.

%\textbf{Organization}. Firstly, we propose the generalized contrastive loss and study its properties (section~\ref{sec:gcl}). Secondly, we construct datasets for studying ``competing features'' in contrastive learning (section~\ref{sec:cf}).

Our main findings and contributions are summarized below.
\begin{itemize}[topsep=0pt, partopsep=0pt, leftmargin=15pt, parsep=0pt, itemsep=5pt]
    % \item We propose a generalized contrastive loss that encapsulates existing contrastive loss as a special case, and compare its various variants.
    \item We propose a generalized contrastive loss, and show that differences between contrastive losses are small with a deep projection head.
    \item We show that the instance-based objective widely used in existing contrastive learning methods can learn on images with multiple objects, and also learn meaningful local features despite operating on global image representation.
    \item We construct three datasets with explicit and controllable competing features to systematically study the feature suppression effect in contrastive learning.
    \item We show that a few bits of easy-to-learn shared features can suppress, and even fully prevent, the learning of other sets of competing features. In scenarios where there are multiple objects in an image, the dominant object would suppress the learning of smaller objects. This poses open challenges to existing contrastive learning.
\end{itemize}


==> content/related.tex <==
\section{Related Work}
Our work studies the contrastive loss based on cross entropy loss~\cite{sohn2016improved,oord2018representation,wu2018unsupervised,chen2020simple}. This loss is widely used in recent successful contrastive learning methods~\citep{oord2018representation,wu2018unsupervised,hjelm2018learning,bachman2019learning,henaff2019data,tian2019contrastive,misra2019self,he2019momentum,li2020prototypical,tian2020makes,chen2020simple,chen2020big}. In terms of the contrastive loss, our work is perhaps most related to~\cite{wang2020understanding}, which shows that formulating contrastive loss as alignment and uniformity in the hypersphere gives similar performance as the standard contrastive loss. We further generalize this factorization, and show other distribution matching losses can be used, and they could achieve similar results. Other than standard contrastive loss that directly utilize negative examples, BYOL ~\cite{grill2020bootstrap} demonstrates another way to maintain representation distribution/entropy without directly relying on distribution matching, and SWAV~\cite{caron2020unsupervised} shows clustering-based method equipped with proper data augmentations could also achieve similar performance. We conduct preliminary experiments of BYOL on RandBit and found that it also suffers from feature suppression as generalized contrastive loss. It is expected that SWAV would exhibit similar behaviors on RandBit as those random bits could fuel representations for perfect clustering. %Although we do not test these methods directly in this work, we believe likely they also share similar properties as generalized contrastive loss, and also heavily rely on data augmentations to flavor certain set of features than others.

The connection between contrastive loss and mutual information has been studied before~\cite{oord2018representation,poole2019variational}. We show that for the generalized contrastive loss, it can also be related to mutual information. Despite the connection between contrastive loss and mutual information, it has been pointed out that mutual information estimation may suffer from certain limitations~\cite{mcallester2020formal,song2019understanding}. Moreover,~\cite{tschannen2019mutual,tian2020makes} show that higher mutual information learned by the network does not warrant better representation quality. In our work, we find adding mutual information bits between two views which are irrelevant to downstream tasks can be harmful for the quality of learned representations. Data augmentation plays an important role at favoring certain bits of mutual information than others.

There is a growing number of recent work on the topic of understanding contrastive learning, both theoretically~\cite{arora2019theoretical,tsai2020demystifying,tosh2020contrastive,tian2020understanding,lee2020predicting} and empirically~\cite{wang2020understanding,tian2020makes,zhao2020makes,purushwalkam2020demystifying}. However, little work has been done to study the phenomenon of feature suppression. To our knowledge, we are the first one to quantitatively and systematically study this problem. We believe this is still a very open question and could benefit from more future investigation. Finally, the feature suppression effect in unsupervised contrastive learning that we study in this work may also exist in standard supervised learning (``contrastive loss'' between examples and class labels), as suggested by~\cite{hermann2020shapes,shah2020pitfalls}, though the specific form would be different.


==> content/study_lossproj.tex <==
\section{Generalized contrastive loss and differences among its instantiations}
% \section{Differences among generalized contrastive losses are small with a deep projection head}
\label{sec:gcl}

The common contrastive loss used in most recent work is based on cross entropy~\cite{sohn2016improved,oord2018representation,wu2018unsupervised}. Following the notation in~\cite{chen2020simple}, the contrastive loss can be defined between two augmented views $(i, j)$ of the same example for a mini-batch of size of $n$, and can be written as the following.

\begin{equation}
\small
\label{eq:nt_xent}
    \mathcal{L}^{\mathrm{NT}\text{-}\mathrm{Xent}} = -\frac{1}{n}\sum_{i,j\in \mathcal{MB}}\log \frac{\exp(\mathrm{sim}(\bm z_i, \bm z_j)/\tau)}{\sum_{k=1}^{2n} \one{k \neq i}\exp(\mathrm{sim}(\bm z_i, \bm z_k)/\tau)}
\end{equation}

where $\bm z_i, \bm z_j$ are hidden representations of two augmented views of the same example; $\mathrm{sim}(\bm u, \bm v)=\bm u^T \bm v/(\|\bm u\|\|\bm v\|)$ is the cosine similarity between two vectors; $\tau$ is a temperature scalar and $\mathcal{MB}$ is a randomly sampled mini-batch consisting of augmented pairs of images. 
%As shown in~\cite{chen2020simple}, the normalization and temperature scaling play an important role in the quality of learned representations, different from a standard cross entropy loss in supervised learning. 
In~\cite{chen2020simple}, a MLP \textit{projection head} is introduced between intermediate layer $\bm h$ (e.g. output of ResNet encoder) and final output $\bm z$. It is shown that the projection head is very beneficial and $\bm h$ is a much better feature representation than $\bm z$.

In this work, we generalize the standard contrastive loss to the following form.
%Inspired by and built upon~\cite{wang2020understanding}, we propose the following \textit{abstract} form of generalized contrastive loss.

\begin{equation}
\label{eq:gc}\boxed{
\mathcal{L}_{\text{generalized contrastive}} = \mathcal{L}_{\text{alignment}} + \lambda \mathcal{L}_{\text{distribution}
}}\end{equation}
~

Both terms are defined on hidden representations. $\mathcal{L}_{\text{alignment}}$ encourages representations of augmented views to be consistent, while $\mathcal{L}_{\text{distribution}}$ encourages representations (or a random subset of them) to match a prior distribution (of high entropy). It is not difficult to see that the standard contrastive loss in Eq.~\ref{eq:nt_xent} is a special case as it can be re-written as follows (scaled by a constant $\tau$).

\begin{equation}
\small
\label{eq:nt_xent_scaled}
\begin{aligned}
    \tau\mathcal{L}^{\mathrm{NT}\text{-}\mathrm{Xent}} = \underbrace{-\frac{1}{n}\sum_{i,j}\mathrm{sim}(\bm z_i, \bm z_j)}_\text{\normalsize $\mathcal{L}_{\text{alignment}}$}
    +  \underbrace{\frac{\tau}{n}\sum_i\log\sum_{k=1}^{2n} \one{k \neq i}\exp(\mathrm{sim}(\bm z_i, \bm z_k)/\tau)}_\text{\normalsize $\mathcal{L}_{\text{distribution}}$}
\end{aligned}
\end{equation}

This form of factorization in Eq.~\ref{eq:nt_xent_scaled} has been proposed in~\cite{wang2020understanding}, 
where the second $\mathrm{LogSumExp}$ term is referred to as \textit{uniformity} since it encourages representation to uniformly distributed in the hypersphere.
Different from~\cite{wang2020understanding}, here we generalize the hypersphere uniform distribution and study a wider set of prior distributions for their effectiveness in learning representations.
%Although the $\mathrm{LogSumExp}$ and the uniform hypersphere prior are widely used, partially due to the popularity of cross entropy loss, here we are interested in knowing \textit{whether or not it is essential to the effectiveness of contrastive loss}. Are there other priors that could also work (e.g. those in Figure~\ref{fig:prior_example})? And how much difference does it make by using other priors?
% We are interested in knowing if it is essential to use a uniform hypersphere prior for the effectiveness of contrastive loss. Are there other priors that could also work well? And how much difference does it make by using other priors?

%To support more flexible prior distribution, we replace the $\mathrm{LogSumExp}$ term in Eq.~\ref{eq:nt_xent_scaled} with a Sliced Wasserstein Distance (SWD) between representations and the given prior. The details of the formulation and SWD algorithm can be found in appendix \ref{app:gloss}, and different priors we consider are summarized in Table~\ref{tab:gloss_comp}.

\paragraph{SWD for supporting diverse prior distributions.} One issue of using more diverse set of priors is we \textit{cannot} rely on $\mathrm{LogSumExp}$ for matching the distribution. To this end, we resort to the theory of optimal transport, via Sliced Wasserstein Distance (SWD)~\cite{rabin2011wasserstein,bonneel2015sliced,kolouri2019generalized}. For two sets of equal-sized samples from two 1-D distributions, the optimal transport can be obtained by computing two permutations that order the values of both sets of samples respectively. The 1-D Wasserstein distance can then be computed with $\ell_2$ distance between the ordered values. For n-D distributions, we first project the samples to $n$ randomly-generated orthogonal 1-D subspaces, and then compute the sum of 1-D Wasserstein distance across all 1-D subspaces. By adjusting the network weights to minimize the SWD, we are able to reduce the mismatch between the distribution of hidden vectors and a known prior distribution. The detailed algorithm can be found in Algorithm~\ref{alg:swd}.
With SWD loss, we are able to use a wider set of priors, and
%, including those in Figure~\ref{fig:prior_example}, and potentially more.
Table~\ref{tab:gloss_comp} summarizes instantiations of the generalized contrastive loss with different prior distributions and distribution matching loss.
\begin{algorithm}[!t]
\caption{\label{alg:swd} Sliced Wasserstein Distance (SWD) loss.}
\begin{algorithmic}
    \STATE \textbf{input:} activation vectors $\bm H\in\mathbb{R}^{b\times d}$, a prior distribution (e.g. Gaussian) sampler $\mathcal{S}$
    %\vspace{0.5em}
    \STATE draw prior vectors $\bm P\in\mathbb{R}^{b\times d}$ using $\mathcal{S}$
    \STATE generate random orthogonal matrix $\bm W\in \mathbb{R}^{d\times d'}$
    \STATE make projections: $\bm H^{\perp} = \bm H\bm W; \bm P^{\perp} = \bm P\bm W$
    \STATE initialize SWD loss $\ell = 0$
    \FOR{$j \in \{1, 2, \cdots, d'\}$}
         %\STATE $h = \mathrm{sort}(\bm H^{\perp}_{:,j})$
         %\STATE $p = \mathrm{sort}(\bm P^{\perp}_{:,j})$
         \STATE $\ell = \ell + \|\mathrm{sort}(\bm H^{\perp}_{:,j})-\mathrm{sort}(\bm P^{\perp}_{:,j})\|^2$
    \ENDFOR
    \STATE \textbf{return} $\ell / (dd')$
\end{algorithmic}
\end{algorithm}

\begin{table*}[!t]
\centering
\small
\caption{\label{tab:gloss_comp} Instantiations of the generalized contrastive loss, i.e. $\mathcal{L}_{\text{alignment}} + \lambda \mathcal{L}_{\text{distribution}}$, that we use in this work. $\tilde{\bm z}$ denotes $\ell_2$-normalized $\bm z\in \mathbb{R}^d$, and is only used for uniform hypersphere prior.}
\begin{tabular}{ccc}
  \toprule
  \textbf{$\mathcal{L}_\text{align}$} & \textbf{Prior distribution} & \textbf{$\mathcal{L}_\text{distribution}$}  \\ \midrule
  $\frac{1}{nd} \sum_{i,j} \|\tilde{\bm z}_i-\tilde{\bm z}_j\|^2$ & Uniform hypersphere & $\frac{1}{n}\sum_i \log\sum_{j} \exp(\tilde{\bm z_i}^T \tilde{\bm z_j}/\tau)$     \\ \midrule %\frac{1}{n} between \log\sum_{j} 
  $\frac{1}{nd} \sum_{i,j}\|\tilde{\bm z}_i-\tilde{\bm z}_j\|^2$  & Uniform hypersphere & SWD($\tilde{Z}, Z^{prior}$)     \\ \midrule 
  $\frac{1}{nd} \sum_{i,j}\|\bm z_i-\bm z_j\|^2$  & Uniform hypercube & SWD($Z, Z^{prior}$)     \\ \midrule 
  $\frac{1}{nd} \sum_{i,j}\|\bm z_i-\bm z_j\|^2$  & Normal distribution & SWD($Z, Z^{prior}$)     \\
  \bottomrule
\end{tabular}
\end{table*}

\paragraph{Connection with mutual information.} The connection between the standard contrastive loss and mutual information has been shown before~\cite{oord2018representation,poole2019variational}, where the contrastive loss (a.k.a. InfoNCE loss~\cite{oord2018representation}) is shown to be a lower bound of the mutual information. %However, with the generalized contrastive loss, do we still have a similar connection?
To connect the generalized contrastive loss to mutual information, we start by the definition of mutual information between two latent variables $U, V$, which is $I(U; V) = H(U) - H(U|V)$.
% \begin{equation*}
% \label{eq:mi}
% I(U; V) = H(U) - H(U|V)
% \end{equation*}
Comparing this factorization of mutual information with generalized contrastive loss, it is not difficult to see that: 1) the alignment term $\mathcal{L}_{\text{alignment}}$ is directly related to $H(U|V)$ which aims to reduce uncertainty of the other views given one view of the example; and 2) the distribution matching term $\mathcal{L}_{\text{distribution}}$ can be considered as a proxy to $H(u)$ for maximizing the entropy in the representation.
%In particular, for representation in the hypersphere, the entropy is maximized if they are uniformly distributed~\cite{wang2020understanding}. 
It is perhaps worth noting that different from mutual information, the generalized contrastive loss (Eq.~\ref{eq:gc}) allows a tunable weight ($\lambda$) between the alignment and distribution matching term. %, whose relation with the temperature ($\tau$) in standard contrastive loss (Eq.~\ref{eq:nt_xent}) will be discussed later.
The weighting scalar $\lambda$ is (inversely) related to the temperature $\tau$ (details in Appendix~\ref{app:tau_lambda}).

\begin{figure*}[t]
    \centering
    \begin{subfigure}{.32\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{figures/comploss_cifar10_proj=2.pdf}
      \caption{CIFAR-10 (2 layers)}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{figures/comploss_imagenet_proj=2.pdf}
      \caption{ImageNet (2 layers)}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{figures/comploss_imagenet_proj=3.pdf}
      \caption{ImageNet (3 layers)}
    \end{subfigure}
    \caption{\label{fig:comploss_linear}Linear evaluation accuracy of ResNet-50 trained with different losses on CIFAR-10 and ImageNet datasets.
    Numbers of projection head layers are in parentheses. Differences between variants of generalized contrastive loss are small with a deep projection head. Decoupled NT-Xent loss is introduced in~\ref{app:tau_lambda}. Numerical results can be found in Appendix~\ref{app:linear_eval}.}
\end{figure*}

\paragraph{Comparing different instantiations of generalized contrastive loss.} Here we ask: Is it essential to use a uniform hypersphere prior for the effectiveness of contrastive loss? How much differences does it make when different generalized contrastive losses are used? To answer this question, we conduct experiments following SimCLR settings~\cite{chen2020simple,chen2020big}, and use the linear evaluation protocol. Detailed experimental setup can be found in appendix~\ref{app:gloss_setup}.

Figure~\ref{fig:comploss_linear} shows linear evaluation results of models trained with different losses under different training epochs. On CIFAR-10, we see little differences in terms of linear evaluation for variants of the generalized contrastive losses, especially when trained longer than 200 epochs. As for ImageNet, there are some discrepancies between different losses, but they disappear when a deeper 3-layer non-linear projection head is used.

\begin{wraptable}{r}{0.62\textwidth}
    \centering
    \small
    %\vspace{-1.0em}
    \caption{\label{tab:linear_eval_num_imagenet}Linear eval accuracy of ResNet-50 on ImageNet.}
    \begin{tabular}{cc|rrrr}
    \toprule
          \multirow{2}{*}{Projection head}          &       \multirow{2}{*}{Batch size}   & \multicolumn{4}{c}{Epoch}  \\
     &   &     100 &   200 &   400 &   800 \\
    \midrule
    \multirow{3}{*}{2 layers} & 512  &  65.4 &  67.3 &  68.7 &  69.3 \\
                              & 1024 &  65.6 &  67.6 &  68.8 &  69.8 \\
                              & 2048 &  65.3 &  67.6 &  69.0 &  70.1 \\
    \midrule
    \multirow{3}{*}{3 layers} & 512  &  66.6 &  68.4 &  70.0 &  71.0 \\
                              & 1024 &  66.8 &  68.9 &  70.1 &  70.9 \\
                              & 2048 &  66.8 &  69.1 &  70.4 &  71.3 \\
    \midrule
    \multirow{3}{*}{4 layers} & 512  & 66.8 & 68.8 & 70.0 & 70.7 \\
                              & 1024 & 67.0 & 69.0 & 70.4 & 70.9 \\
                              & 2048 & 67.0 & 69.3 & 70.4 & 71.3 \\
    \bottomrule
    \end{tabular}
    \vspace{-1.0em}
\end{wraptable}

Furthermore, we find that deep projection head not only reduces the differences among different generalized contrastive losses, but has a similar effect for batch size. With proper learning rate scaling across batch sizes (e.g. square root scaling with LARS optimizer~\cite{you2017large}), the impact of batch size on representation quality is small. Table~\ref{tab:linear_eval_num_imagenet} demonstrate this phenomenon for the standard contrastive loss, and more results on other losses can be found in Appendix~\ref{app:linear_eval}.

==> content/study_objpart.tex <==
\section{Instance-based objective can learn on images with multiple objects and learn good local features}

Most existing contrastive learning methods~\cite{chen2020simple,he2019momentum,grill2020bootstrap,wu2018unsupervised} define their objectives at the instance level where each image is encoded into a single vector representation (e.g. representations of two random crops of the same image instance are treated as a positive pair). In other words, the objective operates on a global representation of its input rather than on some local regions (of its input).
%This sometimes is also referred as instance discrimination. 
We pose two questions regarding instance-based global objective: 1) when there is only a single (dominant) object in the image, the objective seems reasonable as it encourages the model to learn features relevant to object class, but when there are multiple objects present in the image, can instance-based objective still learn well? 2) Since the instance-based objective uses a global summary of its input, can it still learn good local features (e.g. parts of an object, or multiple objects in the same scheme)? To answer these questions, we use SimCLR as representative for the instance-based objective.

\subsection{SimCLR can learn on images with multiple objects}

Commonly used self-supervised learning datasets, such as MNIST, CIFAR-10, ImageNet, are object centered, i.e. the image is mainly occupied by a single (dominant) object. To experiment with multiple objects in a controllable setting, we propose a new dataset setting by composing multiple digits as follows.

\textbf{MultiDigits dataset}. 
%To control experiments with multiple objects, we construct a probing dataset by randomly placing multiple MNIST digits on the same canvas. 
We place MNIST digits ($28\times28$ size) on a shared canvas ($112\times112$ size). We vary the number of digits placed on the canvas. One factor that could interfere with learning of multiple digits is overlapping digits, therefore we use two placement strategies: random vs in-grid (Figure \ref{fig:probe_data_multidigit}). Random placement of digits incurs no constraint on where digits can be placed on the canvas, whereas in-grid placement puts each digit in one of the $4\times4$ grid cells the canvas is divided into, and no two digits can fall in the same cell. In-grid placement ensures no overlapping of digits.

We first pretrain a ResNet-18 with SimCLR or supervised learning with the same augmentation policy (random cropping and resize) 
%and batch size of 1024. 
on MultiDigits dataset.
%SimCLR models are trained for 400 epochs and supervised models for 100 epochs. 
To access the representation quality, we then train linear classifiers for images with a single digit of size $28\times28$ on the canvas. Similarly during evaluation, we place only one digit of size $28\times28$ on the canvas.

As shown in Table \ref{tab:multidigit}, representations learned using supervised loss maintains its quality when up to 8 digits are placed in the image. After that the representation becomes worse as the canvas gets more crowded. Notably, representations learned using SimCLR display a similar phenomenon. Regardless of placement strategy, top-1 accuracy stays at the same level up to 8 digits, demonstrating that SimCLR can learn from images with multiple objects. In addition, the increased performance gap between the two placement strategies with increased number of digits shows that object overlapping makes it harder for contrastive losses to learn from multiple objects.

\begin{figure*}[!t]
    \centering
    \begin{subfigure}{.495\textwidth}
      \centering
      \includegraphics[width=0.95\linewidth]{figures/d4_random.pdf}
      \caption{4 digits, random placement.}
    \end{subfigure}
    \begin{subfigure}{.495\textwidth}
      \centering
      \includegraphics[width=0.95\linewidth]{figures/d16_random.pdf}
      \caption{16 digits, random placement.}
    \end{subfigure}
    \begin{subfigure}{.495\textwidth}
      \centering
      \includegraphics[width=0.95\linewidth]{figures/d4_ingrid.pdf}
      \caption{4 digits, in-grid placement.}
    \end{subfigure}
    \begin{subfigure}{.495\textwidth}
      \centering
      \includegraphics[width=0.95\linewidth]{figures/d16_ingrid.pdf}
      \caption{16 digits, in-grid placement.}
    \end{subfigure}
    \caption{\label{fig:probe_data_multidigit}MultiDigit dataset. More digits lead to more overlapping in random placement.}
\end{figure*}

\begin{table*}[h]
\centering
\small
\caption{\label{tab:multidigit} Top-1 linear evaluation accuracy (\%) for pretrained ResNet-18 on the MultiDigits dataset.
We vary the number of digits placed on the canvas during training from 1 to 16. During evaluation only 1 digit is present.
As a baseline, a network with random weights gives 18\% top-1 accuracy.}
\begin{tabular}{llcccccc}
  \toprule
   & Placing of digits & \multicolumn{6}{c}{Number of digits (size $28\times28$)} \\
   & & 1 & 2 & 4 & 8 & 12 & 16 \\
  \midrule
  \multirow{2}{*}{Supervised} & Random & 99.5 & 99.5 & 99.3 & 99.4 & 98.9 & 98.3 \\
             & In-grid & 99.5 & 99.6 & 99.5 & 99.3 & 98.6 & 92.4 \\
  \midrule
  \multirow{2}{*}{SimCLR} & Random & 98.9 & 98.9 & 99.0 & 98.9 & 98.2 & 96.4 \\
             & In-grid & 98.3 & 98.6 & 99.1 & 99.2 & 99.1 & 98.3 \\
  \bottomrule
\end{tabular}
\end{table*}

\subsection{SimCLR learns local features that exhibit hierarchical properties}

To understand the local features learned by SimCLR, we apply K-means on intermediate features of the pretrained ResNet with SimCLR, and see how local regions of an image are grouped together. For good representations, we expect that regions of similar objects or object parts should be grouped together.

Specifically, we take a pretrained Resnet-50 $2\times$ 
%with selective kernels 
on ImageNet, and run inference on images (from ImageNet validation set and COCO~\cite{lin2014microsoft}) of size 448$\times$448. We run K-means with various numbers of clusters on the l2-normalized hidden features from middle layers of the network (e.g. block group 2,3,4 of the ResNet). We also compare SimCLR learned features with supervised learned features, as well as the raw pixel (RGB) features extracted from each $14\times14$ patch.

\begin{figure*}[!t]
    \centering
    \begin{subfigure}{.495\textwidth}
      \centering
      \includegraphics[width=0.99\linewidth]{figures/local_inet_dog_bi}
      \caption{\label{fig:vis_local_parts_a}Features from different methods.}
    \end{subfigure}
    \begin{subfigure}{.495\textwidth}
      \centering
      \includegraphics[width=0.99\linewidth]{figures/local_inet_dog_bg_bi}
      \caption{\label{fig:vis_local_parts_b}SimCLR features at different ResNet layers.}
    \end{subfigure}
    \caption{\label{fig:vis_local_parts}Visualizing features on a ImageNet validation image with K-means clustering. Each row denotes a type of local features used, and each column denotes the number of K-means clusters. 
    Later layers of SimCLR/supervised ResNet tend to group by object parts.
    More visualization examples can be found in \href{https://contrastive-learning.github.io/intriguing}{https://contrastive-learning.github.io/intriguing}.
    }
\end{figure*}

Figure~\ref{fig:vis_local_parts_a} shows that as the number of clusters increases, the learned representations tend to group image regions based on parts of the object (i.e. facial components of the dog). This phenomenon appears in both SimCLR and supervised learned features, but not with raw pixel features, indicating meaningful local features learned by SimCLR and supervised learning. In Figure~\ref{fig:vis_local_parts_b}, we compare ResNet intermediate features at different layers, and it suggests that earlier layers contain more edge-related features, while later layers contain more object/part features.

\begin{figure*}[!t]
    \centering
    \begin{subfigure}{.495\textwidth}
      \centering
      \includegraphics[width=0.99\linewidth]{figures/local_coco_meet_bi}
      \caption{}
    \end{subfigure}
    \begin{subfigure}{.495\textwidth}
      \centering
      \includegraphics[width=0.99\linewidth]{figures/local_coco_room_bi}
      \caption{}
    \end{subfigure}
    \caption{\label{fig:vis_local_multi_objs}Visualizing features on two images from COCO. Each row denotes a type of local features (SimCLR, Supervised, and raw pixels; both SimCLR and Supervised are trained on ImageNet), and each column denotes the number of K-means clusters. Region grouping by SimCLR/supervised features tend to overlap with object class.}
\end{figure*}

Figure~\ref{fig:vis_local_multi_objs} show region grouping results on two COCO images of SimCLR and supervised learning (trained on ImageNet). Again, region grouping by local features tend to overlap with object class, indicating good local features learned.

